HalluciDoctor: Mitigating Hallucinatory Toxicity in Visual Instruction Data

Multi-modal Large Language Models (MLLMs) tuned on machine-generated instruction-following data have demonstrated remarkable performance in various multi-modal understanding and generation tasks. However, the hallucinations inherent in machine-generated data, which could lead to hallucinatory outputs in MLLMs, remain under-explored. This work aims to investigate various hallucinations (i.e., object, relation, attribute hallucinations) and mitigate those hallucinatory toxicities in large-scale machine-generated visual instruction datasets. Drawing on the human ability to identify factual errors, we present a novel hallucination detection and elimination framework, HalluciDoctor, based on the cross-checking paradigm. We use our framework to identify and eliminate hallucinations in the training data automatically. Interestingly, HalluciDoctor also indicates that spurious correlations arising from long-tail object co-occurrences contribute to hallucinations. Based on that, we execute counterfactual visual instruction expansion to balance data distribution, thereby enhancing MLLMs' resistance to hallucinations. Comprehensive experiments on hallucination evaluation benchmarks show that our method successfully mitigates 44.6% hallucinations relatively and maintains competitive performance compared to LLaVA. The data and code for this paper are publicly available. \url{https://github.com/Yuqifan1117/HalluciDoctor}.

==> sec/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}

% Multi-modal Large Language Models~(MLLMs) aim to mimic human perception of the world and help humans better understand the world. 
Recently, Multi-modal Large Language Models~(MLLMs) have made promising progress on multi-modal tasks, such as image captioning, visual question-answering, and visual conversations~\cite{tsimpoukelli2021multimodal, li2022blip, li2023blip, alayrac2022flamingo}. Additionally, inspired by the impressive instruction-following capability of LLMs~\cite{touvron2023llama, chiang2023vicuna, peng2023instruction}, several more powerful MLLMs~\cite{liu2023visual, zhu2023minigpt, ye2023mplug, dai2023instructblip, li2023empowering} have recently emerged, extending instruction-tuning to the multimodal space. Due to the scarcity of visual-language instruction-following data, recent research\cite{liu2023visual, zhu2023minigpt} presents a data reformation approach, which leverages text-only LLMs conditioned on image captions and bounding boxes to create instruction-following data involving visual content.
\begin{figure}[!t]
    \centering
    \includegraphics[width=1.\linewidth]{figures/example-2.pdf}
    \caption{(a) On the top, we show an example of visual instruction data and various kinds of hallucinations in it. (b) On the bottom, we report the MME performance and the extended CHAIR of MLLMs~(\textsl{i.e.}, MiniGPT-4) to show the hallucinatory toxicity.} 
    \vspace{-4mm}
    \label{hallucination-example}
\end{figure}
However, since these visual instructions are generated by text-only LLMs, they may contain hallucinatory responses that conflict with the image content. For instance, as shown in Figure~\ref{hallucination-example}.a, the response in the visual instruction data includes object hallucinations such as ``a few traffic lights" and relation hallucinations like ``people gathered for flying kites" instead of ``sitting and watching". These hallucinatory responses may compromise the MLLM's ability to accurately perceive the real world. 

% When we systematically analyze the hallucinatory toxicity of the visual instruction dataset generated by ChatGPT/GPT-4, we find that previous hallucination elimination methods largely neglect the inconsistent descriptions in the visual instruction datasets.

Motivated by this insight, we systematically definite various types of hallucinations~(\textsl{i.e.}, object, relation, attribute hallucinations) and investigate them in visual instruction datasets. Using the widely used dataset LLaVA-Instruction-158K~\cite{liu2023visual}, we employ the extended CHAIR metrics to conduct comprehensive evaluations of the impact of these visual instruction data on modern MLLMs, considering both performance and hallucination issues. We observe that fine-tuning the LLaVA data leads to improved MLLM performance, but there is a noticeable increase in the probability of hallucinations~(Figure~\ref{hallucination-example}.b, left vs. middle). These observations confirm with recent studies~\cite{liu2023aligning, gunjal2023detecting, li2023evaluating}, which show that current machine-generated instruction-following data itself contains massive pernicious hallucinations. This pushes us to focus on dispelling hallucinatory toxicity in it.

Previous works mainly focus on collecting extra remedial training data~\cite{liu2023aligning, wang2023vigc, lu2023evaluation} or utilize additional plug-in models~\cite{gunjal2023detecting, yin2023woodpecker, liao2023revo} to mitigate the hallucinations during inference. LRV-Instruction~\cite{liu2023aligning} proposes to add extra negative instructions to increase the robustness of the MLLM against hallucinations. M-HalDetect~\cite{gunjal2023detecting} mitigates hallucinations by incorporating an additional trained reward model during the inference phase. These methods are time-consuming. Furthermore, they only superficially suppressed the hallucinatory output of MLLM, largely neglecting the existing hallucinatory toxicity in the visual instruction dataset generated by ChatGPT/GPT-4. This leads to suboptimal hallucination elimination.

% After eliminating the hallucinations in LLaVA, the probability of hallucinations is greatly reduced while keeping the performance of MLLM improved~(Figure~\ref{hallucination-example}.b, middle vs. right)
In contrast to the aforementioned methods, we aim to eradicate hallucinations in machine-generated visual instruction data. The primary challenge is how to automatically detect various kinds of hallucinations from massive instruction tuning data without the need of manual annotations. For this, we propose a flexible Hallucination Detection and Elimination Framework, \textbf{HalluciDoctor}, which automatically detects various hallucinations in arbitrary positions and dispels them based on a cross-checking paradigm. The key insight of HalluciDoctor is that when asked about the hallucinatory content of a given image, the responses from different MLLM experts typically tend to vary and can even contradict each other. Following it, HalluciDoctor breaks the hallucination detection procedure into four sub-processes: 1) \textit{Answer Chunks Extraction}: extract all answer chunks including objects, attributes, and relations by textual scene graph parsing as description-oriented answers; 2) \textit{Answer-based Question Generation}: generate corresponding fine-grained questions for each answer chunk with various types; 3) \textit{Consistency Cross-Checking}: obtain candidate image-oriented answers from multiple MLLMs and cross-check the consistency between description-oriented answer chunks and their corresponding image-oriented answers. Subsequently, HalluciDoctor identifies those semantic chunks whose consistency scores are below the threshold as hallucinatory chunks and accurately eliminates those hallucinations in visual instructions without destroying the semantics of context.

In our exploration to eliminate hallucinations of visual instructions, we find that the cross-checking information from HalluciDoctor not only helps to locate hallucinations but also contains other most relevant contents, which frequently co-occur with the hallucinatory items. Empirically, the long-tail distribution of co-occurrence leads MLLMs to produce hallucinatory outputs based on spurious associations rather than the actual content in the image.

the elements that frequently co-occur with those confusing contents are often the most challenging samples for MLLMs to accurately distinguish. Motivated by concepts in causal learning, we attempt to use HalluciDoctor to provide disturbed guidance to form counterfactual instructions and utilize Stable Diffusion~\cite{hertz2022prompt, brooks2023instructpix2pix} to generate corresponding aligned images with minimal editing. Training MLLMs with counterfactual instruction samples introduces a robust inductive bias, mitigating the risk of learning spurious correlations within visual instruction data. This enhances MLLM's ability to recognize confusing samples and resist hallucinations. To sum up, our main contributions are summarized as follows:
\begin{itemize}
    \item To the best of our knowledge, we are the first to comprehensively investigate the severe hallucination toxicity in existing machine-generated visual instruction datasets.
    \item We propose a novel \textbf{HalluciDoctor} method to detect various hallucinations by a consistency cross-checking paradigm and dispel them in a low-resource way.
    \item Based on HalluciDoctor, we further automatically generate more counterfactual instruction data to improve the MLLM's resistance to hallucinations.
    \item Our empirical study confirms the effectiveness of our method in eliminating various hallucinations in visual instruction data and improving MLLMs' robustness.

\end{itemize}




 

 


%-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}

Our proposed methodology for automatically identifying and eliminating hallucinations in the visual instruction data~(\textit{e.g.}, LLaVA). First, given an image-instruction-response pair in the dataset, we extract all answer chunks from instructions and responses as description-oriented answers. Second, guided by the context and those extracted answers, we generate corresponding questions with various types assisted with LLM. Third, each generated question is fed to MLLM experts to generate corresponding image-oriented answers as candidate answers. Subsequently, we will conduct cross-checks for consistency between candidate answers and semantically-aligned question-answer pairs to determine the presence of hallucinatory phrases in the sentences. Fourth, we can comprehensively eliminate detected hallucinatory items with better visual instruction alignment through inconsistency chunks removal and counterfactual sample generation.
\begin{figure*}
  \centering
    \includegraphics[width=1.\linewidth]{figures/framework-2.pdf}
  \caption{Our proposed methodology for automatically identifying and eliminating hallucinations in the visual instruction data~(\textit{e.g.}, LLaVA). First, given an image-instruction-response pair in the dataset, we extract all answer chunks from instructions and responses as description-oriented answers. Second, guided by the context and those extracted answers, we generate corresponding questions with various types assisted with LLM. Third, each generated question is fed to MLLM experts to generate corresponding image-oriented answers as candidate answers. Then we will perform the consistency cross-checking between candidate answers and semantic-aligned Q-A pairs to ascertain whether the sentence contains hallucinatory phrases. Fourth, we can comprehensively eliminate detected hallucinatory items with better visual instruction alignment through inconsistency chunks removal and counterfactual sample generation.}
  \label{framework}
\end{figure*}


==> sec/2_related_work_old.tex <==
\section{Related works}
\label{relatedworks}

\subsection{Large Vision-Language Model} 
% Due to the scaling up of training data and an increase in the number of parameters, 
In recent years, large language models~(LLMs) have shown remarkable performance in a zero-shot/few-shot setting~\cite{zhao2023survey}, such as performing user instruction following~\cite{ouyang2022training, li2023otter}, complex reasoning~\cite{wei2022chain, yao2023tree}, and in-context learning~\cite{rubin2021learning, wang2022self}. Inspired by this, there has been notable interest in integrating powerful LLMs into pre-trained vision-language models for challenging vision-language tasks~\cite{tsimpoukelli2021multimodal, li2023blip, yu2023visually, guo2023images}. More recently, some multi-modal large language models~(MLLMs)~\cite{liu2023visual, zhu2023minigpt, ye2023mplug, dai2023instructblip, li2023empowering, bai2023qwen} have emerged to better emulate human perceptual capabilities and show excellent generalization performance in unseen VL tasks. Generally, an MLLM aligns a vision encoder into an advanced language model through a cross-modal alignment network~(\textit{e.g.}, a linear projection layer in LLaVA~\cite{liu2023visual} and MiniGPT-4~\cite{zhu2023minigpt}, visual abstractor in mPLUG-Owl~\cite{ye2023mplug}). The training process of MLLMs mainly contains two major stages. The first stage aims to acquire vision-language knowledge by pretraining the model on large-scale aligned image-text pairs. In the second stage, the pre-trained model is finetuned on the curated multi-modal instruction datasets to enhance its conversation ability as a chatbot. Once the visual encoder and the LLM are well-aligned, MLLMs exhibit excellent visual understanding ability for various multimodal tasks.

\subsection{MLLM Hallucination}
Although LLMs have demonstrated remarkable performances in various tasks, they still suffer from hallucinations that give deviated answers for nonexistent knowledge. \cite{zhang2023siren} summarizes three main hallucination types contained in LLMs that hinder the steady use of LLMs in real-world deployment. Since MLLMs are built on LLMs, they also suffer from the hallucination inherited from LLMs.
% ~(\textsl{i.e.}, input-conflicting hallucination, context-conflicting hallucination, and fact-conflicting hallucination). 
Moreover, MLLMs suffer image inconsistency issues where the response is inconsistent with the target image or the input instructions. Commonly used image captioning evaluation metrics such as CIDEr and SPICE lack precise penalties for hallucination occurrences, while conventional CHAIR needs manually defined rules for exact matching. Therefore, it is necessary to design a specific detection method for MLLM hallucination. \cite{li2023evaluating} explores object hallucinations in MLLMs by classifying the existence of arbitrary objects, but ignoring elaborate hallucinations~(\textit{e.g., attribute hallucinations and relation hallucinations}) in the visual instruction data. \cite{liu2023aligning} prevents hallucinations by introducing negative instructions for robust instruction tuning and \cite{gunjal2023detecting} attempts to address hallucinations during inference through a reward model. Unlike existing studies that ignore the alignment of images and instructions in the process of detecting and repairing hallucinations, we design a comprehensive detection framework for diverse types of hallucinations. This framework addresses hallucinations and broadens the data distribution at both visual and linguistic levels.

\subsection{Synthetic Data for Visual Tasks}
Recently, text-to-image diffusion models have achieved remarkable performance on image generation tasks~\cite{ramesh2022hierarchical,rombach2022high,saharia2022photorealistic}, which has stimulated strong interest in the domain of data augmentation with synthetic images~\cite{lin2023explore, he2022synthetic, yu2023interactive, trabucco2023effective}. 
% \cite{he2022synthetic} use GLIDE~\cite{nichol2021glide} to generate class-conditioned images and explore the effectiveness of synthetic data for image recognition. 
% \cite{lin2023explore} performs image pasting with synthetic data to obtain label images containing unseen targets, improving performance for few-shot object detection. 
However, existing text-to-image models require longer and more complex prompts to yield impressive outcomes. Notably, \cite{le2023coco} makes minimal counterfactual changes to image text with more concise text-controlled image editing~\cite{hertz2022prompt, brooks2023instructpix2pix} for improving out-of-domain generalization of multimodal vision-language models. Our method differs from prior work as it emphasizes minimal compositional changes for the image instruction data to increase MLLM's resistance to hallucinatory errors. 


==> sec/3_method_old.tex <==
\section{The Toxicity of Visual Instruction Data}
Due to the scale limitation of multimodal instruction-following data, there is a growing interest in self-generated instructions for multimodal large language models~\cite{liu2023visual, zhu2023minigpt}. However, as ChatGPT generates these visual instructions, they are susceptible to containing hallucinations themselves and will mislead MLLM to generate hallucinatory content not depicted in the image. To our knowledge, we are the first work to analyze the hallucinatory toxicity of auto-generated visual instruction data systematically.
\subsection{Hallucination Metrics}
\label{metric}
To better analyze hallucinatory toxicity in visual instruction data, we first systematically define three types of hallucinations frequently appearing in the dataset: 1) \textit{object hallucination} are those objects that appear in the description but not the image. 2) \textit{relation hallucination} involves relations among corresponding objects that exhibit inconsistencies between the description and the image. 3) \textit{attribute hallucination} refers to inaccurate object properties in the description, such as size, color, and states. 

The current popular metric CHAIR~\cite{rohrbach2018object} only calculates the proportion of nonexistent objects in the description. Thus, we extend the naive CHAIR metric into more complex scenarios to evaluate various kinds of hallucinations. Initially, we incorporate synonym lists into annotated objects and phrases, forming an enhanced ground truth set. Subsequently, we split the description into sentences and extracted all objects, relations, and attributes for a comprehensive assessment. The extended CHAIR metric then calculates the ratio of sentences containing hallucinatory elements not present in the image. Accordingly, the definition of extended CHAIR, including ${\rm CHAIR}_{obj}$, ${\rm CHAIR}_{rel}$, and ${\rm CHAIR}_{attri}$, is delineated as follows:
% Specifically, the automatic CHAIR first identifies all objects, relations, and attributes in the description. Subsequently, it utilizes labeling tools~\cite{kirillov2023segment} to form a ground truth set for object existence assessment. 
% Subsequently, it identifies all objects, relations, and attributes in the description and computes the proportion of all elements that are not present in the image. To systemically evaluate all kinds of hallucinations in the visual instructions, we extend CHAIR to CHAIR++, which computes ${\rm CHAIR}_{obj}$, $\rm{CHAIR}_{act}$, and ${\rm CHAIR}_{attri}$ for various hallucinations as follows:
\begin{eqnarray}
\tiny
    {\rm CHAIR}_{obj} = \frac{|\rm{\{SENT\ with\ nonexistent\ object\}}|}{|\rm{\{all \quad SENT\}}|}
\end{eqnarray}
\begin{eqnarray}
\tiny
    {\rm CHAIR}_{rel} = \frac{|\rm{\{SENT\ with\ nonexistent\ relation\}}|}{|\rm{\{all\quad SENT\}}|}
\end{eqnarray}
\begin{eqnarray}
    {\rm CHAIR}_{attri} = \frac{|\rm{\{SENT\ with\ nonexistent\ attribute\}}|}{|\rm{\{all\ SENT\}}|}
\end{eqnarray}
where SENT denotes each sentence in the description and the higher CHAIR score indicates there exists more hallucinations. Notably, we compute the ${\rm CHAIR}_{rel}$ and the ${\rm CHAIR}_{attri}$ only among existent objects to avoid misjudging compositional errors influenced by object hallucinations as additional hallucination errors.
\subsection{Hallucinatory Toxicity Statistics}
Utilizing our extended CHAIR metric designed for in-depth hallucination analysis, we meticulously examine the hallucination frequency within machine-generated visual instruction data. We concentrate on prevalent, machine-generated visual instruction datasets, namely LLaVA~\cite{liu2023visual} and MiniGPT4-Instruction~\cite{zhu2023minigpt}.
% Considering the scalability and generality of the data, we mainly analyze the hallucination statistics of auto-generated visual instruction data. 
LLaVA consists of 158K distinct instruction-following samples generated by GPT-4, while MiniGPT4-Instruction includes about 3.5K instances refined by ChatGPT from detailed descriptions.

To tackle the challenge of incomplete annotation in large-scale visual instruction datasets, particularly regarding relations and attributes, we have employed a proxy assessment utilizing powerful visual foundation models to reflect the hallucinatory toxicity.
 
One major challenge that makes the evaluation more difficult than prior studies~\cite{li2023evaluating} is that we lack ground truth labels for exact matching in large-scale visual instruction data, particularly for relations and attributes. To partly reflect the severity of hallucinations in visual instruction data, we use powerful visual foundation models to provide proxy assessments. We adopt an object detector GroundingDINO~\cite{liu2023grounding} to annotate objects and use the image-text similarity of BLIP~\cite{li2022blip} to judge the existence of relations and attributes. Subsequently, we use these pseudo-labels to calculate all CHAIR results and compare them to the upper bound result from MSCOCO annotations. As illustrated in Table~\ref{hallucination_statistics}, all types of hallucinations in MiniGPT-4 and LLaVA, especially object hallucinations, exhibit much more occurrence than in human annotations, reflecting the seriousness of the hallucination issue in the dataset. 

However, this method relies on the accuracy of annotations and is inflexible to detect a wide range of hallucinations. Therefore, we propose a general hallucination detection and elimination framework \textbf{HalluciDoctor} based on the consistency cross-checking paradigm to handle the potential hallucinations in the training data.

\begin{table}[t]
\resizebox{0.47\textwidth}{!}{
\centering
\begin{tabular}{lccccc}
\hline
\toprule
Dataset & \#Samples & ${\rm CHAIR}_{obj}$ & ${\rm CHAIR}_{rel}$ & ${\rm CHAIR}_{attri}$ & Length\\ \hline
MSCOCO~\cite{lin2014microsoft} & 118K &4.0& 2.4 & 3.1 & 46.4 \\\hline
MiniGPT-4~\cite{zhu2023minigpt}& 3.5K & 68.5 & 16.3 & 26.3 & 70.8 \\
LLaVA~\cite{liu2023visual} & 158K & 76.9 & 32.1 & 24.3 & 96.1 \\ 
LLaVA+ & 158K &  &  &  &  \\ 

\bottomrule
\end{tabular}
}
\caption{The statistics of three types of hallucinations in visual instruction data and comparison with ground truth from MSCOCO.}
\vspace{-5mm}
\label{hallucination_statistics}
\end{table} 



\section{HalluciDoctor Framework}
As illustrated in Figure~\ref{framework}, our approach \textbf{HalluciDoctor} involves a three-step process. Initially, we probe hallucinations using a cross-checking paradigm. Subsequently, we eliminate hallucinatory errors through LLM. Finally, we expand the visual instruction data by generating counterfactual samples, thus enhancing the robustness of MLLM. We will elaborate on the details in the following subsections.
% We first analyze the toxicity of hallucinations in the LLaVA dataset by experimental results and then introduce our hallucination detection pipeline. 
% We will elaborate on how to eliminate hallucinations in visual instructions in Section~\ref{session4}.
\subsection{Hallucination Cross-Checking Paradigm}
% need to focus on the hallucination
\label{CCF_1}
% Upon analyzing the toxicity of the synthetic visual instructions, we deem it essential to detect and eliminate extensive hallucinations within it. 
% Although we have examined the toxicity of hallucinations in visual instruction data, it is non-trivial to identify and eliminate hallucinations without manual annotations or extra evidence. Moreover, abstract hallucinatory errors further complicate the process of hallucination detection. Therefore, we extract unlabeled semantic units by question-answering and design a consistency-checking paradigm to automatically detect various hallucinatory errors. 

\noindent\textbf{Overview.} To exhaustively identify various types of hallucinations~(\textsl{i.e.}, object hallucinations, relation hallucinations, attribute hallucinations) in the corresponding description of each image, we introduce a hallucination cross-checking paradigm. Our insight is to decompose this demanding detection task into several simpler answer consistency-checking tasks. This paradigm comprises four subtasks: answer chunks generation, question generation, consistency cross-checking, and hallucination elimination. 

% . When the description-oriented answer is inconsistent with multiple image-oriented candidate answers, it suggests that there is a potential hallucination between the description and the image content. Concretely, we break down the whole process into four subtasks: answer chunks generation, question generation, consistency cross-checking, and hallucination elimination 

% Concretely, given an image $I$ with its instruction-following data~($\rm{X}_q, \rm{X}_a$), where $\rm{X}_q$ is the instruction from human and $\rm{X}_a$ is the corresponding response from GPT-4. We concatenate the instruction $\rm{X}_q$ and its response $\rm{X}_a$ as a total sequence $S$. Then we extra semantic units $\{a_{t,1},...,a_{t,n}\}$ from $S$ as description-oriented answers and generate corresponding questions $\{q_{t,1},...,q_{t,n}\}$. For all generated questions, we will use MLLM experts to obtain image-oriented candidate answers $\{\{a_{t,1}^1, a_{t,1}^2, a_{t,1}^3\},...,\{a_{t,n}^1, a_{t,n}^2, a_{t,n}^3\}\}$. Here, $n$ denotes the number of semantic chunks and $a_{t,n_i}^n$ denotes one candidate answer based on the image content. We will identify which semantic unit $a_{t,n_i}$ is contradictory to its candidate answers $\{a_{t,n_i}^1, a_{t,n_i}^2, a_{t,n_i}^3\}$ as hallucinations.

\noindent\textbf{Answer Chunks Generation.} Since descriptions contain massive concepts in one sentence, we initially extract massive answer chunks including objects, attributes, and relationships in the generated sentence to completely represent the whole sentence. Given an image $I$ with its instruction-following data~($\rm{X}_q, \rm{X}_a$), where $\rm{X}_q$ is the instruction from human and $\rm{X}_a$ is the corresponding response from GPT-4. We concatenate $\rm{X}_q$ and $\rm{X}_a$ together as a total sentence $S$ for answer chunk generation. Then we extra all answer chunks from $S$ as description-oriented answers as follows,
\begin{equation}
   A_S =\{a_{1},...,a_{n}\}
\end{equation}
where $n$ denotes the number of all answer chunks. This step is crucial for subsequent evaluation results.

\noindent\textbf{Question Generation.} After producing answer chunks, we generate questions that will be later used to derive image-oriented candidate answers for consistency checking. These questions are generated based on the relevant context and corresponding answer chunks. We employ LLM like ChatGPT as potent question generators to encompass the wide diversity of semantic chunks and diverse question types. Thus, we can generate a range of questions tailored to different types of answers, including concrete objects, abstract relationships, and attribute descriptions. We denote the corresponding questions of the sentence $S$ as follows,
\begin{equation}
   Q_S =\{q_{1},...,q_{n}\}
\end{equation}
\noindent\textbf{Consistency Cross-Checking.} The consistency cross-checking step aims to verify the consistency between each answer chunk $a_i$ and its corresponding content in the image. 
To obtain the specific image content, we use the generated questions to derive image-oriented candidate answers based on MLLM experts~(\textit{e.g.}, BLIP2~\cite{li2023blip}, InstructBLIP~\cite{dai2023instructblip}, and MiniGPT-4~\cite{zhu2023minigpt}). Formally, let $\{\mathcal{F}_x\}_{x=1,2,3}$ denote MLLM experts, the prompt template slotted with the reference image $I$ and one question $q_i$ is fed to the MLLM $\mathcal{F}_x$ to produce the image-oriented candidate answer $a_i^x=\mathcal{F}_x(I,q_i)$.  Once we collect image-oriented candidate answers $\{a_i^x\}_{x=1,2,3}$ for each answer chunk $a_i$, we will compare the consistency between them. We employ a Bert-based metric~(\textsl{i.e.}, BEM~\cite{bulian2022tomayto}) to evaluate the consistency since this metric provides more flexibility in the answer formulation than strictly hard matching. 
Let $\mathcal{B}(\cdot,\cdot|q)$ denote the BEM score between two answers according to the question, the final \textit{ConScore} of the answer chunk $a_i$ is calculated by voting as follows,
\begin{equation}
    ConScore_i = \frac{1}{m}\sum_{x=1}^m\mathcal{B}(a_i,a_i^x)
\end{equation}
where $m$ represents the number of MLLM experts for evaluation. We will consider the answer chunk $a_i$ as a hallucination when its ConScore is $\textless$ 0.5. This process helps us ascertain whether the current description accurately describes factual information in the image.

% After thoroughly examining the existence of hallucinations in the visual instruction data, it is crucial to eliminate the detected hallucinations for better alignment between images and instructions. Current approaches to hallucination elimination primarily focus on scaling up high-quality instruction data through manual correction~\cite{} or training additional hallucination revisers to correct hallucinatory captions~\cite{gunjal2023detecting, liu2023aligning}. However, these works require task-specific training data with time-consuming collection, making them impractical for hallucination elimination in large-scale synthetic visual instructions.
 % Since the visual instruction data contains serious hallucination errors, it is crucial to eliminate the detected hallucinations. However, current approaches require time-consuming data collection to train task-specific models for detecting and preventing hallucinations in MLLMs~\cite{gunjal2023detecting, liu2023aligning}, making them impractical for hallucination elimination in large-scale synthetic visual instructions. 

\noindent\textbf{Hallucination Elimination.} Benefits from the above subtasks, we can accurately locate hallucinatory chunks with their contexts. Subsequently, we employ an LLM to automatically remove the hallucinatory chunks based on the context and guarantee the coherence and harmony of the corresponding sentences. Following this recovery process, we acquire faithful visual instructions with reduced hallucinatory descriptions and more consistent responses, intended to mitigate the hallucinatory toxicity of machine-generated visual instruction data during MLLM training.
% We categorize hallucinations into two types: ``strict hallucinations" when candidate answers are consistent, and ``ambiguous hallucinations" when candidate answers exhibit inconsistency. We eliminate the description associated with strict hallucinations and incorporate human verification for ambiguous hallucinations to further rectify the descriptions. This results in aligned visual instruction data with fewer hallucinations. Notably, human validation can be readily substituted with powerful GPT-4V~\cite{gpt4v} to minimize overhead. accurately identify hallucinatory descriptions within specific semantic chunks.
\begin{table*}[!t]
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{lclccc|cccc}
\hline
\toprule
&\multirow{2}{*}{Backbone} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Instance-level} &\multicolumn{3}{c}{Sentence-level}&\multirow{2}{*}{Avg Len} \\\cline{4-6} \cline{7-9}
& &  & {\rm CHAIR}_{obj} \downarrow & {\rm CHAIR}_{rel} \downarrow &{\rm CHAIR}_{attri} \downarrow &{\rm CHAIR}_{obj} \downarrow & {\rm CHAIR}_{rel} \downarrow &{\rm CHAIR}_{attri} \downarrow &\\\hline
\multirow{10}{*}{\rotatebox[]{90}{MS-COCO}} 
&\multirow{5}{*}{MiniGPT4~(7B)} & Original & 6.8& 3.4 &4.6&11.3 &7.1&9.3&65.9 \\
& & w/ LLaVA & 19.3 & 9.1 &3.4& 39.2 &24.4&10.9&86.4\\ 
& & w/ LRV & 14.3 & 7.8& 6.1& 22.2 &14.4&15.3&72.2\\ 
& & w/ LLaVA+ & 14.0&6.4&3.4&29.2 &21.5& 9.6& 88.6\\
& & w/ LLaVA++ & &&& &&& \\\cline{2-10}
&\multirow{5}{*}{mPLUG-OWL~(7B)} & Original  &18.4  & 19.2& &33.3&&27.3 & 50.3 \\
& & w/ LLaVA & & &&&& & \\ 
& & w/ LRV && &&&& &  \\ 
& & w/ LLaVA+ & & &&&  &&\\ 
& & w/ LLaVA++ & & &&&  &&\\ 
\bottomrule
\end{tabular}
}
\caption{CHAIR evaluation results to show the recovery effect of hallucinatory elimination of HalluciDoctor on MLLM.}
\label{hallucination_chair}
\end{table*} 

\subsection{Seesaw-based Visual Instruction Expansion}
\label{CCF_3}
In the realm of MLLMs, the frequently co-occurring object groups~(\textit{e.g.}, chair, room, and clock) often result in spurious correlations that affect the output~\cite{li2023evaluating, zhou2023analyzing}. In our efforts to locate hallucinations, we have noticed the context of various hallucinations often contains their frequently co-occurring objects. We attribute this phenomenon to the spurious correlation stemming from the long-tail distribution of object co-occurrence in visual instruction data. 
% Therefore, we create counterfactual samples by adding hallucinatory content to infrequent scenarios and balance visual instructions through these counterfactual samples to reduce the impact of spurious correlations. However, selecting the target scenario has two conflicting challenges: a) the local augmentation of tail co-occurrence objects; and b) the global plausibility of infrequent scenes. 
Hence, we introduce counterfactual generation for visual instructions to reduce the impact of spurious correlations. However, it is non-trivial to create suitable counterfactual visual instructions due to the complexity of the target scene for various hallucinations. To this end, we propose a seesaw-based strategy with an augmented factor and an inhibiting factor to adaptively select the target scenario for counterfactual generation.

\noindent\textbf{Augmented Factor.} 
% The augmented factor aims to balance the co-occurrence of all classes with hallucinatory content by adjusting the weight of tail objects, shown as follows,
The augmented factor aims to enhance the weight of infrequent objects, and its value is negatively correlated with the number of co-occurrences, shown as follows,
\begin{equation}
    \mathcal{A}_{ij}=\left\{
	\begin{array}{ccc}
		\frac{n_i}{\max(n_j,1)}      &  ,   & \rm{if}\ {n_j\leq n_i}\\
		1    &  ,   & \rm{if}\ {n_j>n_i}\\ 
	\end{array}\right.~.
\end{equation}
where $n_i$ denotes the number of co-occurrences between the hallucination $a_i$ and its most relevant content $C_i$ in the context, while $n_j$ denotes the number of co-occurrences of other tail objects and the hallucination. 

\noindent\textbf{Inhibiting Factor.} Although the augmented factor effectively enhances the co-occurrence of tail classes, it may encourage irrational tail predictions due to excessive counterfactual intervention. Therefore, we propose the inhibiting factor to suppress the weights of tail objects that are infrequent co-occurring with the context as follows,
\begin{equation} 
    \mathcal{I}_{ij}=\left\{
	\begin{array}{ccc}
		\frac{m_j}{m_i}    &  ,   & \rm{if}\ {m_j\leq m_i}\\ 
                1      &  ,   & \rm{if}\ {m_j>m_i}\\
	\end{array}\right.~.
\end{equation}
where $m_i$ is equal to $n_i$ and $m_j$ represents the number of co-occurrences of tail objects and the most relevant content $C_i$ aforementioned. Once we obtain $\mathcal{A}_{ij}$ and $\mathcal{I}_{ij}$, we calculate the seesaw score for all co-occurring objects of each hallucination $a_i$ as shown below,
\begin{equation} 
    \rm{SeesawScore}_{ij}=\mathcal{A}_{ij}*\mathcal{I}_{ij}~.
\end{equation}

In the counterfactual generation process, we select the scene containing the object with the highest seesaw score as the target scenario and add the hallucinatory content to the target scenario to get a counterfactual caption. Subsequently, we use SAM~\cite{kirillov2023segment} to obtain image masks for minimal image editing and use instruction-based image editing models~\cite{brooks2023instructpix2pix, hertz2022prompt} to generate instruction-aligned counterfactual images. The generated counterfactual pairs are then combined with the recovered LLAVA dataset to form the more robust dataset LLaVA++, thereby reducing the influence of spurious correlations on hallucination generation. Please refer to Appendix C for more details.

 

%a diffusion-based inpainting model~\cite{brooks2023instructpix2pix} is used to modify the causal terms in the corresponding image to achieve congruence with the generated counterfactual samples. Notably, we only select the mask of the replaced part using SAM~\cite{kirillov2023segment} for minimal image editing, guaranteeing the aligned semantics of the visual instructions remain unaltered. 
 

 

 

 

 

% Our proposed methodology for automatically identifying and eliminating hallucinations in the visual instruction data. First, given an image-instruction pair in the LLaVA, we generate corresponding scene graphs from sentence-level conversations and extract semantic answer chunks by enumerating all information units in scene graphs. Second, conditioned on the context guidance and each extracted answer from conversations, corresponding questions with diverse types are generated by LLM. Third, each semantic-aligned question-reference pair with its context from the original dataset is then fed to other multimodal model experts to produce relevant candidate answers. Once we get candidate answers for specific context-question-reference pairs, we evaluate answer consistency by statistical distance, thus judging hallucination existence based on the consistency score. Fourth, we can employ LLMs to analyze associative terms of hallucinations in context and obtain casual candidates based on co-occurrence relevance to generate counterfactual samples. Finally, the detected hallucination is automatically repaired by removing contradictions based on consistency, and the distribution of related elements is extended by counterfactual samples based on AI-generative methods.









 

% One approach for detecting hallucinations involves utilizing established intrinsic uncertainty metrics like token probability or entropy~\cite{manakul2023selfcheckgpt, fu2023gptscore}. These metrics explicitly show the most uncertain part of the system's output sequence, where hallucinations are more prone to occur. 

==> sec/4_experiments_old.tex <==
\section{Experiments}
\label{session4}

\subsection{Implementation Setup}
\noindent\textbf{Datasets.} MSCOCO~\cite{lin2014microsoft} is a comprehensive dataset with 80 object categories used for diverse vision tasks. Visual Genome ~\cite{krishna2017visual} is another vision dataset with more detailed visual information like bounding boxes and region captions. In this paper, we utilize LLaVA-158k~\cite{liu2023visual}, which contains images from MSCOCO, as visual instruction data to verify the effectiveness of our framework. Following previous works~\cite{liu2023aligning, li2023evaluating}, we randomly select 500 unique images from the intersection of COCO 2014 and Visual Genome for a more detailed evaluation. Notably, these images were different from the ones used in LLaVA-158k~\cite{liu2023visual} and contained various annotations~(\textsl{i.e.}, objects, relations, and attributes) for evaluating all kinds of hallucinations.

\noindent\textbf{\textcolor{red}{Evaluation Benchmarks.}} \textbf{CHAIR} is dedicated to evaluating the hallucinatory toxicity of visual instruction data and the hallucination of MLLMs. Apart from the above CHAIR evaluation at the sentence level~(\textsl{i.e.}, ${\rm CHAIR}_S$), we also assess the hallucination of MLLMs at the instance level~(\textsl{i.e.}, ${\rm CHAIR}_I$) by counting all nonexistent instances within a sentence. Following the setting in session \ref{metric}, we prompt MLLMs with the instruction of \texttt{Provide a detailed description of the given image} to generate detailed captions. Notably, we enforce the continued generation of short captions to ensure that captions are detailed enough for a fair comparison. We then compute the ${\rm CHAIR}_S$ and ${\rm CHAIR}_I$ scores for all types of hallucinations by referencing the ground truth. 

\textbf{MME}~\cite{fu2023mme} is a public benchmark to evaluate the perception and cognition abilities of MLLMs on 14 subtasks. This setup transforms human annotations into a series of ``Yes-or-No" questions and measures the performance of MLLMs by summing the answer accuracy for each subtask. In this paper, we compute the total score of the MME in cognition and perception for all models, where a higher score means better performance and fewer hallucinations of the MLLM.

To strike an optimal balance between reducing hallucinations and delivering detailed descriptions, we have incorporated GPT-4 evaluations to assess the accuracy and variety in MLLM-generated descriptions of MSCOCO images comprehensively. We employ GPT-4 to assess MLLMs, quantifying both the prevalence of hallucinations and the granularity of detail in their descriptions. \textbf{OwlEval}~\cite{ye2023mplug} is another visually-related evaluation set with 82 artificially constructed questions. We manually score these responses from all models on a 3-0 quality scale~(corresponding to A-D in the official setup) and compute a total score to assess the open domain capability of MLLMs.
% We manually score 50 single-turn responses given by all models to evaluate the open domain capabilities of MLLMs.


\noindent\textbf{Models.} The comparison models include: \textit{Original}, which directly uses the pre-trained model from the first stage without any other visual instruction dataset finetuning; \textit{w/ LLaVA}, which is finetuned on full LLaVA dataset~\cite{liu2023visual}; \textit{w/ LRV}, which instruct-tunes the backbone on LRV-Instruction~\cite{liu2023aligning}; \textit{w/ LLaVA+}, which is fine-tuned on the refined LLaVA after hallucinatory elimination of HalluciDoctor; \textit{w/ LLaVA++}, which performs instruction-tuning on the extended LLaVA+ data after the counterfactual sample expansion by HalluciDoctor. We integrate the above methods into two popular MLLM backbones: (1) MiniGPT-4~\cite{zhu2023minigpt}; (2) mPLUG-OWL~\cite{ye2023mplug} to evaluate the effectiveness of hallucination elimination and MLLMs' performance.

\noindent\textbf{Training Details.} As for MiniGPT4, we initialize from its checkpoint of the first pretraining stage and only fine-tune the linear projection layer of the model for 10 epochs. As for mPLUG-Owl, we train the text encoder with the LoRA strategy and train for 3 epochs. Due to limited computing resources, we set the batch size to 4 and only fine-tuned the 7B model with NVIDIA RTX 3090. Additionally, we only change the corresponding instruction data under different settings, and keep other parameters the same as the original model to make a fair comparison in our experiments.


\subsection{Comparion of MLLM Hallucinations}
In this section, we compare our MLLMs with HalluciDoctor against the above baseline models. We follow the standard pipeline of CHAIR~\cite{rohrbach2018object} to perform automated computations of ${\rm CHAIR}_{obj}$, ${\rm CHAIR}_{rel}$, and ${\rm CHAIR}_{attri}$ at two different levels and report the total results in Table~\ref{hallucination_chair}.
Based on the observation of experimental results, we have summarized the following conclusions:

\textbf{Visual instruction data has serious hallucinatory toxicity.} We compare the MLLM with LLaVA to the original MLLM. It can be seen that MLLMs are more prone to produce hallucinations after instruction-tuning on the LLaVA dataset, especially in object perception. This confirms our previous analysis of visual instruction data, emphasizing the necessity for eliminating the pronounced hallucinatory toxicity within the dataset.

\textbf{Our HalluciDoctor can be flexibly equipped to
different MLLMs for hallucination elimination.} We utilize HalluciDoctor to eliminate hallucinations and generate counterfactual samples in LLaVA, resulting in the refined LLaVA+ and LLaVA++, respectively. We integrate these refined datasets into two backbone models, namely MiniGPT-4~\cite{zhu2023minigpt} and mPLUG-OWL~\cite{ye2023mplug}, for the evaluation of hallucinations. Despite the model diversity, MLLMs with LLaVA+ can consistently reduce the probability of various hallucinations~(xx\%/xx\%/xx\% in MiniGPT-4 and xx\%/xx\%/xx\% in mPLUG-owl for object/relation/attribute hallucinations). Moreover, MLLMs fine-tuned on LLaVA++ both achieve more reductions in most hallucination metrics, which indicates that the expansion of visual instruction data can eliminate the hallucinatory impact of spurious correlations derived from the object co-occurrence. 

\textbf{Compared with other model-agnostic methods, our
HalluciDoctor outperforms in both instance-level and sentence-level hallucination elimination.} Specifically, LLaVA+ exceeds the SOTA of the hallucination elimination model LRV-Instruction~\cite{liu2023aligning} for all three types of hallucinations with consistent improvements~(xx\% v.s. xx\% for object hallucinations). It shows that our HalluciDoctor can reduce massive hallucinations in the visual instruction data to achieve better instruction alignment, which is conducive to improving the stability of the MLLMs. Moreover, we notice that MLLM with LLaVA+ still suffers from object hallucinations, suggesting that MLLM may incorrectly fit some illusory characteristics in the training set. In contrast, MiniGPT-4 equipped with the counterfactual sample expansion LLaVA++ shows fewer hallucinations, especially for object hallucinations. This suggests that the alignment of counterfactual samples enhances the ability of MLLMs to discern between distinct objects, thereby refining their perception of detailed scene information.
% Moreover, the MiniGPT-4 fine-tuned on the refined LLaVA++ from HalluciDoctor produced fewer hallucinations, especially for object hallucinations. This suggests that the alignment of counterfactual samples enhances the ability of MLLMs to discern between distinct objects, thereby refining their perception of detailed scene information.

% It is worth noting that the LLaVA+ of MLLMs not only achieves the fewest hallucinations but also maintains details of the description, while the LRV-Instruction limiting the length of the output results in less detailed descriptions.

\textbf{Our method balances dispelling the MLLM hallucinations and preserving description detailedness.} Empirically, a direct comparison of hallucination frequency is compromised by substantial variation in the average lengths of sentences. Consequently, we extend our evaluation by prompting GPT-4 to conduct a thorough comparison of the detailedness and accuracy of descriptions generated by MLLMs. In Figure~\ref{gpt4_results}, we visualize the result scores of GPT-4 evaluations under different MLLMs, respectively. On the one hand, LLaVA significantly enriches the content of descriptions while increasing hallucinations. On the other hand, LRV-Instruction~\cite{liu2023aligning} reduces such hallucinatory errors but at the expense of narrative diversity, thereby limiting the model's generative potential. In contrast, our HalluciDoctor outperforms other models on a total score, indicating that it is able to eliminate hallucinations while preserving MLLM's ability to output diverse descriptions.

\begin{figure}
  \centering
    \includegraphics[width=1.\linewidth]{figures/gpt4_results.pdf}
  \caption{Evaluation scores of detailedness and accuracy for descriptions from MiniGPT-4 with different setups. We visualized the total scores using an orange line, where higher scores indicate more detailed descriptions and fewer hallucinations.}
  \label{gpt4_results}
\end{figure}
 
\begin{figure*}
  \centering
    \includegraphics[width=1.\linewidth]{figures/visualization.pdf}
  \caption{A case study comparing the levels of MLLM hallucination after fine-tuning on various instruction data.}
  \label{visualization}
\end{figure*}

\subsection{In-depth Analysis}
% 虽然我们提出的CHAIR和GPT-4 evaluation验证了HalluciDoctor消除幻觉的优越性，但是对于其对MLLM性能的影响还缺乏定量的分析
\noindent\textbf{Evaluation on MLLM performance.} Although the proposed CHAIR and GPT-4 evaluation validate the superiority of the hallucinatory elimination of HalluciDoctor, its effect on the performance of MLLMs still lacks a well-rounded analysis. Therefore, we conduct quantitative analysis on MME and OwlEval benchmarks.
We report each model's MME cognitive and perceptual performance in Table~\ref{mme_evaluation}. 
% 我们可以看到，LLaVA+相比于original model也能带来很大的分数提升，即使在更少量的视觉指令数据下也取得了和LRV-Instruction有竞争力的性能，这说明HalluciDoctor消除指令数据中的幻觉同时并没有破坏MLLM的性能。
We can see that LLaVA+ contributes great score improvement compared with the original model and achieves competitive performance compared with LRV-Instruction even with less visual instruction data. This indicates that HalluciDoctor maintains the performance of the MLLM when dispelling various hallucinations.
% 从经验上看，LLaVA++消除了大规模指令数据中的幻觉毒害以及带来更具挑战性的反事实指令，可以实现更好的泛化
In addition, LLaVA++ can bring out more challenging counterfactual instructions for better generalization. With the help of LLaVA++, both fine-tuned MLLMs have been further improved~(+59.32 / +xx.xx in perception and +31.42 / +xx.xx in cognition). 
Qualitatively, we further perform a human evaluation using the OwlEval benchmark and show the visualized results for all MLLMs in Figure~\ref{owleval}.
% 在使用LLaVA++的mllm的情况下，我们观察到在整体长度保持的条件下响应质量有了实质性的改善
In the case of MLLMs with LLaVA++, we observe a substantial improvement in response quality under preserving overall length.
This result demonstrates the capability of HalluciDoctor to effectively improve the response quality with fewer hallucinations, as opposed to roughly limiting the response length.
% Since the questions were open-ended, in our setup, we manually evaluated the model responses for A, B, C, or D metrics based on the effective length of the responses and the quality of the responses, respectively.

 

\begin{table}[!t]
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lclcc}
\hline
\toprule
&Backbone & Method &  Perception & Cognition \\ \hline

\multirow{8}{*}{\rotatebox[]{90}{MME Benchmark}} 
&\multirow{5}{*}{MiniGPT4~(7B)} & Original &  616.41 &  232.71 \\
& & w/ LLaVA~\cite{liu2023visual} & 859.64 & 289.29\\ 
& & w/ LRV~\cite{liu2023aligning} & 895.96 & 296.43\\ 
& & w/ LLaVA+ & 889.32 & 317.86\\
& & w/ LLaVA++ & \textbf{955.28} & \textbf{320.71} \\\cline{2-5}
&\multirow{4}{*}{mPLUG-owl~(7B)} & Original  &  967.34 & 276.07 \\
& & w/ LLaVA & & \\ 
& & w/ LLaVA+ & &\\ 
& & w/ LLaVA++ & &\\ 
\bottomrule
\end{tabular}
}
\caption{Results on MME evaluation~\cite{fu2023mme} of MiniGPT4-7B and mPLUG-Owl-7B. Original denotes without any instructions for fine-tuning and others denote fine-tuned on our refined instruction data, respectively. The performance is measured by the sum of subtasks scores, where the best score for each partition is bolded.}
\label{mme_evaluation}
\end{table} 

% \begin{figure}[!t]

%   \centering
%    \begin{subfigure}{0.495\linewidth}
%     \centering
%     \includegraphics[width=1.\linewidth]{figures/llm_test_score.pdf}
%     \caption{MiniGPT-4 Results}
%     \label{input}
%   \end{subfigure}
%   \begin{subfigure}{0.495\linewidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/llm_test_score.pdf}
%     \caption{mPLUG-OWL Results}
%     \label{sg1}
%   \end{subfigure}
%   \caption{}
%   \label{owleval}
% \end{figure}
\begin{figure}
  \centering
    \includegraphics[width=1.\linewidth]{figures/llm_test_score.pdf}
  \caption{Response quality~(y-axis, higher is better), response length~(x-axis, higher is better), and response stability~(circle sizes, smaller is better) of various MLLMs on the OwlEval benchmark.}
  \label{owleval}
\end{figure}
\noindent\textbf{\textcolor{red}{Analysis of Framework Modules.}} \textcolor{red}{Hallucination-eliminating measures (naive delete or LLM), choice of threshold (0.5), and proportion of counterfactual samples (our is only 2500).}

\noindent\textbf{\textcolor{red}{Robustness Analysis of HalluciDoctor.}} \textcolor{red}{Our method is also applicable to other datasets~(MiniGPT-4) and can also be used to further mitigate hallucinations in the inference stage.}

 

\noindent\textbf{Visualization Results.} 
In Figure~\ref{visualization}, we visualize the process of HalluciDoctor dispelling the hallucinatory toxicity in visual instruction data and present the corresponding case with rectified descriptions.

\section{Conclusions}
In this work, we delve deep into the underlying hallucination phenomena in machine-generated visual instruction data.
% 在这项工作中，我们提出了一个灵活的框架，利用基于问答的交叉验证来自动检测并消除蕴藏在视觉指令数据中的潜在幻觉
We introduce a flexible framework that exploits question-based cross-checking to automatically detect and eliminate potential hallucinations. 
% 在消除幻觉毒害的指令数据和额外的反事实样本的帮助下，我们提升了模型的感知能力，从而解决了MLLM中的幻觉困扰
% We tackle the hallucinatory disturbance with the help of abundant faithful instructions from HalluciDoctor and improve the perception ability of MLLMs based on counterfactual instruction expansion,
% We further identify the co-occurrence issue resulting in hallucinations and enhance MLLM's resistance to hallucinations by counterfactual instruction expansion.
We have additionally pinpointed the co-occurrence issue that leads to hallucinations and augmented the MLLMs' resistance to such errors through counterfactual instruction expansion.
% 自动指标和人工评估的广泛实验结果证明了我们的方法在消除各种幻觉和保留 MLLM 的开放能力方面的优越性。
The extensive experimental results by both automatic metrics and human evaluations demonstrate the superiority of our approach in dispelling various hallucinations and retaining MLLM's open-end capabilities.


